Legal-HNet: Mixing Legal Long-Context Tokens with Hartley Transform

Since its introduction, the transformers architecture has seen great adoption in NLP applications, but it also has limitations. Although the self-attention mechanism allows for generating very rich representations of the input text, its effectiveness may be limited in specialized domains such as legal, where, for example, language models often have to process very long texts. In this paper, we explore alternatives to replace the attention-based layers with simpler token-mixing mechanisms: Hartley and Fourier transforms. Using these non-parametric techniques, we train models with long input documents from scratch in the legal domain setting. We also introduce a new hybrid Seq2Seq architecture, a no-attention-based encoder connected with an attention-based decoder, which performs quite well on existing summarization tasks with much less compute and memory requirements. We believe that similar, if not better performance, as in the case of long correlations of abstractive text summarization tasks, can be achieved by adopting these simpler infrastructures. This not only makes training models from scratch accessible to more people, but also contributes to the reduction of the carbon footprint during training.

==> sections/exluded_tokenizers_study.tex <==
%Study of tokenizers on BillSum Train Set
%mean num characters: 10272.54
%tokenizer                       type        vocab size  mean num tokens     character token ratio   
%bert-base-cased                 WP          29K         2023.09             5.078                   
%bert-base-uncased               WP          31K         1884.24             5.452                   
%albert-base-v2                  Unigram     30K         1935.68             5.307
%google/fnet-base                Unigram     32K         1947.43             5.275
%google/pegasus-large            Unigram     96K         1763.40             5.825                   
%microsoft/deberta-v3-base       Unigram     128K        1838.87             5.586
%ours                            BPE         64K         1909.23             5.380                   
%xlm-roberta-base                BPE         250K        2007.56             5.117                   
%allenai/longformer-base-4096    BPE         50K         3664.36             2.803
%gpt2                            BPE         50K         3664.36             2.803


==> sections/models_overview.tex <==
% \section{Overview of Compared Models}
% \label{sec:models_overview}

% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{llrrrrrrrr}
%     \toprule
%         Model Name & Source & P. Steps (K) & P. BS & \# P. Examples (M) & \# Enc. Params (M) & Max Seq Len & Vocab Size (K) & PubMed Rouge-L & BillSum Rouge-L \\ 
%     \midrule
%         DOC + SUM & \cite{kornilova_billsum_2019} & 1000 & 256 & 256 & 340 & 512 & 30 & ~ & 33.73 \\ 
%         Transformer-base & \cite{zhang_pegasus_2020} & ~ & ~ & ~ & 110 & 1024 & 96 & 19.02 & 30.98 \\ 
%         PEGASUS-base & \cite{zhang_pegasus_2020} & 500 & 256 & 128 & 110 & 1024 & 96 & 25.23 & 37.78 \\ 
%         PEGASUS-large-C4 & \cite{zhang_pegasus_2020} & 500 & 8192 & 4096 & 340 & 1024 & 96 & 27.69 & 45.8 \\ 
% %        BudgetLongformer small caselaw & ours & 100 & 32 & 3.2 & 29 & 4096 & 64 & ~ & 40.22 \\ 
%         BudgetLongformer small diverse & ours & 100 & 32 & 3.2 & 29 & 4096 & 64 & 23.24 & 37.58 \\ 
%         %BudgetLongformer small diverse 1024 -> 128 & ours & 100 & 32 & 3.2 & 29 & 4096 & 64 & 26.03 & 42.50 \\ 
% %        BudgetLongformer base caselaw & ours & 100 & 32 & 3.2 & 159 & 4096 & 64 & ~ & 45.17 \\ 
%         BudgetLongformer base diverse & ours & 100 & 32 & 3.2 & 159 & 4096 & 64 & 26.53 & 40.50 \\ 
%         %BudgetLongformer base diverse 1024 -> 128 & ours & 100 & 32 & 3.2 & 159 & 4096 & 64 & 27.21 & 44.21 \\ 
%     \end{tabular}
% }
% \caption{Abbreviations: P.: Pretraining, BS: Batch Size, Enc.: Encoder, Params: Parameters.
% Comparison of the models evaluated on the summarization tasks BillSum and PubMed.
% }
% \label{tab:summarization_models}
% \end{table*}


% \begin{table*}[t]
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llrrrrrrrrrrr}
%     \toprule
%         Model Name & Source & P. Steps (K) & P. BS & D. Steps (K) & D. BS & WS Steps (K) & WS BS & \# P. Examples (M) \downarrow & \# Params (M) \downarrow & Max Seq Len \uparrow & Vocab Size (K) & LexGLUE Micro-F1 \uparrow \\ 
%     \midrule
%     small models \\
%     \midrule
%         BERT-Tiny & \cite{turc_well-read_2019} & 1000 & 256 & 1400 & 256 & ~ & ~ & 614.4 & 4.4 & 512 & 31 & 70.1 \\ 
%         miniLM & \cite{wang-etal-2021-minilmv2} & 1000 & 256 & 400 & 256 & ~ & ~ & 358.4 & 21 & 512 & 30 & 72.8 \\ 
%         DistilBERT & \cite{sanh_distilbert_2020} & 1000 & 256 & 500 & 256 & ~ & ~ & 384 & 66 & 512 & 30 & 75.2 \\ 
%         LegalBERT-small & \cite{chalkidis_legal-bert_2020} & 1000 & 256 & ~ & ~ & ~ & ~ & 256 & 35 & 512 & 31 & 76.7 \\ 
%         BudgetLongformer small caselaw & ours & 100 & 32 & ~ & ~ & ~ & ~ & 3.2 & 29 & 4096 & 64 & 73.9 \\ 
%         BudgetLongformer small diverse & ours & 100 & 32 & ~ & ~ & ~ & ~ & 3.2 & 29 & 4096 & 64 & 73.4 \\ 
%         \midrule
%         base models \\
%         \midrule
%         BERT & \cite{devlin_bert_2019} & 1000 & 256 & ~ & ~ & ~ & ~ & 256 & 110 & 512 & 30 & 77.8 \\ 
%         RoBERTa & \cite{liu_roberta_2019} & 500 & 8192 & ~ & ~ & ~ & ~ & 4096 & 125 & 512 & 31 & 77.8 \\ 
%         DeBERTa & \cite{he_debertav3_2021} & 1000 & 256 & ~ & ~ & ~ & ~ & 256 & 139 & 512 & 128 & 78.3 \\ 
%         BigBird & \cite{zaheer_big_2021} & 500 & 8192 & ~ & ~ & 500 & 256 & 4224 & 127 & 4096 & 50 & 78.2 \\ 
%         Longformer & \cite{beltagy_longformer_2020} & 500 & 8192 & ~ & ~ & 65 & 64 & 4100.16 & 149 & 4096 & 31 & 78.5 \\ 
%         Legal-BERT-base & \cite{chalkidis_legal-bert_2020} & 1000 & 256 & ~ & ~ & ~ & ~ & 256 & 110 & 512 & 31 & 79.8 \\ 
%         CaseLaw-BERT & \cite{zheng_when_2021} & 2000 & 256 & ~ & ~ & ~ & ~ & 512 & 110 & 512 & 30 & 79.4 \\ 
%         BudgetLongformer base caselaw & ours & 100 & 32 & ~ & ~ & ~ & ~ & 3.2 & 159 & 4096 & 64 & 76.0 \\ 
%         BudgetLongformer base diverse & ours & 100 & 32 & ~ & ~ & ~ & ~ & 3.2 & 159 & 4096 & 64 & 76.9 \\ 
%     \bottomrule
% \end{tabular}
% }
% \caption{Abbreviations: P.: Pretraining, D.: Distillation, WS: Warm Start, BS: Batch Size, Params: Parameters.
% Comparison of the models evaluated on LexGLUE. In cases where we were not able to find the batch size in the papers, we assumed it to be 256, since this is the most widely used batch size in pretraining and the default for BERT. For DistilBERT we were not able to find the number of distillation steps, so we assumed 500K steps.
% %DistilBERT was trained for 90 hours on 8 16GB NVIDIA V100 GPUs. RoBERTa was trained on 1024 32GB NVIDIA V100 GPUs for 500K steps. Our training took 60 hours on 4 16GB NVIDIA V100 GPUs. 
% }
% \label{tab:lexglue_models}
% \end{table*}

% In this section, we show detailed overviews of the model specifics (Tables \ref{tab:summarization_models} and \ref{tab:lexglue_models}).

